Conservative Discrete Structure Stabilizes Autoregressive Rollouts in a 1D Drift Diffusion Poisson Benchmark

Learned plasma transport surrogates can match short horizon states while failing over long rollouts because charge accounting, density admissibility, and Poisson compatible field reconstruction are not enforced. We study this issue in a controlled nondimensional one dimensional drift diffusion Poisson benchmark with Dirichlet electrostatic potential boundaries and zero species wall fluxes. The benchmark is a conservation and rollout test, not a complete sheath wall model. We compare Conservative FluxNet, a structure preserving flux correction model with a conservative finite volume update and positivity aware limiting, against direct next state regressors, direct variants with Poisson recomputation, charge projection, and rollout training, and a classical conservative core without learned correction. The central result is that the classical finite volume core alone achieves near roundoff rollout error, so the paper is primarily about conservative discrete structure rather than learned closure. On the headline experiment, the conservative model achieves rollout MSE $7.35\times 10^{-9}$ versus $4.23\times 10^{1}$ for the unconstrained baseline, $2.53\times 10^{1}$ with Poisson recomputation, $6.72\times 10^{1}$ with charge projection, and $2.71\times 10^{1}$ with four step rollout training. Across $64$ prespecified configurations, it wins rollout mean squared error in $60/64$ cases despite winning one step mean squared error in only $19/64$. These results show that, for this controlled benchmark and comparison class, local conservative finite volume structure is more important than one step neural regression accuracy for stable autoregressive rollout.

==> tables/all_active_evaluations.tex <==
\scriptsize
\begin{longtable}{@{}p{0.32\linewidth}rrrrrrrr@{}}
\caption{Complete active comparative evaluation registry. Abbreviations: Cons., conservative model; Base., direct baseline; CE, rollout charge error.} \label{tab:all_active_evaluations}\\
\toprule
Case & $N_x$ & Steps & Traj. & Eval & Cons. MSE & Base MSE & Cons. CE & Base CE \\
\midrule
\endfirsthead
\toprule
Case & $N_x$ & Steps & Traj. & Eval & Cons. MSE & Base MSE & Cons. CE & Base CE \\
\midrule
\endhead
1. 10 headline & 16 & 64 & 64 & 128 & 7.35e-09 & 42.3 & 5.93e-15 & 4.48 \\
2. 15 multi seed / seed 001 & 16 & 64 & 64 & 128 & 6.56e-09 & 18.9 & 6.49e-15 & 0.358 \\
3. 15 multi seed / seed 002 & 16 & 64 & 64 & 128 & 6.14e-09 & 58.4 & 3.57e-15 & 2.22 \\
4. 15 multi seed / seed 003 & 16 & 64 & 64 & 128 & 7.19e-09 & 29.1 & 8.75e-15 & 2.72 \\
5. 15 multi seed / seed 004 & 16 & 64 & 64 & 128 & 1.19e-08 & 19.6 & 6.86e-15 & 0.257 \\
6. 15 multi seed / seed 005 & 16 & 64 & 64 & 128 & 7.05e-09 & 95.9 & 8.11e-15 & 1.27 \\
7. 18 harder regimes / bias stronger & 16 & 64 & 64 & 128 & 7.82e-09 & 12.5 & 4.20e-15 & 1.45 \\
8. 18 harder regimes / data sparse & 16 & 64 & 8 & 128 & 1.32e-08 & 49.6 & 4.48e-15 & 8.84 \\
9. 18 harder regimes / long horizon sparse & 16 & 64 & 8 & 256 & 1.19e-07 & 485 & 1.60e-14 & 113 \\
10. 18 harder regimes / stiff transport & 16 & 96 & 32 & 160 & 7.20e-09 & 54.7 & 6.50e-15 & 0.954 \\
11. 19 core ablation / classical core only & 16 & 64 & 64 & 128 & 1.15e-14 & 42.3 & 6.88e-15 & 4.48 \\
12. 19 core ablation / correction scale small & 16 & 64 & 64 & 128 & 2.50e-10 & 42.3 & 1.11e-14 & 4.48 \\
13. 20 stability / rollout 016 & 16 & 64 & 64 & 16 & 2.34e-11 & 0.0122 & 9.92e-16 & 4.86e-04 \\
14. 20 stability / rollout 032 & 16 & 64 & 64 & 32 & 1.36e-10 & 0.276 & 1.89e-15 & 0.0203 \\
15. 20 stability / rollout 064 & 16 & 64 & 64 & 64 & 9.62e-10 & 4.27 & 2.95e-15 & 0.522 \\
16. 20 stability / rollout 128 & 16 & 64 & 64 & 128 & 7.35e-09 & 42.3 & 5.93e-15 & 4.48 \\
17. 23 learned value v2 / teacher flux classical core only v2 & 8 & 64 & 64 & 128 & 0.0406 & 1.56 & 1.09e-14 & 0.77 \\
18. 23 learned value v2 / teacher flux formal v2 & 8 & 64 & 64 & 128 & 0.0404 & 1.56 & 1.63e-14 & 0.77 \\
19. 23 learned value v2 / teacher flux positivity stress classical core only v2 & 8 & 64 & 64 & 128 & 0.212 & 0.96 & 2.23e-14 & 0.436 \\
20. 23 learned value v2 / teacher flux positivity stress formal v2 & 8 & 64 & 64 & 128 & 0.207 & 0.96 & 2.10e-14 & 0.436 \\
21. 31 generalization v2 / bias mild & 8 & 64 & 64 & 128 & 0.0216 & 0.45 & 1.47e-14 & 0.0955 \\
22. 31 generalization v2 / bias strong & 8 & 64 & 64 & 128 & 0.0713 & 3.72 & 1.44e-14 & 2.39 \\
23. 31 generalization v2 / dt large & 8 & 64 & 64 & 128 & 0.0796 & 1.56 & 1.29e-14 & 0.77 \\
24. 31 generalization v2 / dt small & 8 & 64 & 64 & 128 & 0.0146 & 1.58 & 1.70e-14 & 0.77 \\
25. 31 generalization v2 / electron diffusivity high & 8 & 64 & 64 & 128 & 0.0517 & 1.67 & 7.93e-15 & 0.77 \\
26. 31 generalization v2 / electron diffusivity low & 8 & 64 & 64 & 128 & 0.0212 & 1.41 & 1.38e-14 & 0.77 \\
27. 31 generalization v2 / electron mobility high & 8 & 64 & 64 & 128 & 0.0735 & 1.5 & 1.36e-14 & 0.77 \\
28. 31 generalization v2 / electron mobility low & 8 & 64 & 64 & 128 & 0.023 & 1.67 & 8.11e-15 & 0.77 \\
29. 31 generalization v2 / ion diffusivity high & 8 & 64 & 64 & 128 & 0.0423 & 1.57 & 1.03e-14 & 0.77 \\
30. 31 generalization v2 / ion diffusivity low & 8 & 64 & 64 & 128 & 0.0407 & 1.56 & 1.41e-14 & 0.77 \\
31. 31 generalization v2 / ion mobility high & 8 & 64 & 64 & 128 & 0.0923 & 1.55 & 8.35e-15 & 0.77 \\
32. 31 generalization v2 / ion mobility low & 8 & 64 & 64 & 128 & 0.0327 & 1.57 & 2.24e-14 & 0.77 \\
33. 41 mesh resolution v2 / grid 008 & 8 & 64 & 64 & 128 & 0.0404 & 1.56 & 1.63e-14 & 0.77 \\
34. 41 mesh resolution v2 / grid 016 & 16 & 64 & 64 & 128 & 0.119 & 14.2 & 4.04e-15 & 1.48 \\
35. 41 mesh resolution v2 / grid 032 & 32 & 64 & 64 & 128 & 0.459 & 13.4 & 1.32e-14 & 0.245 \\
36. 41 mesh resolution v2 / grid 064 & 64 & 64 & 64 & 128 & 0.704 & 10.3 & 9.04e-15 & 0.0948 \\
37. 51 data regime v2 / trajectories 004 & 8 & 64 & 4 & 128 & 0.0404 & 8.76 & 2.09e-14 & 0.561 \\
38. 51 data regime v2 / trajectories 008 & 8 & 64 & 8 & 128 & 0.0401 & 12.6 & 9.20e-15 & 8.32 \\
39. 51 data regime v2 / trajectories 016 & 8 & 64 & 16 & 128 & 0.0401 & 28.8 & 1.20e-14 & 0.375 \\
40. 51 data regime v2 / trajectories 032 & 8 & 64 & 32 & 128 & 0.0402 & 2.03 & 9.36e-15 & 0.739 \\
41. 51 data regime v2 / trajectories 064 & 8 & 64 & 64 & 128 & 0.0404 & 1.56 & 1.63e-14 & 0.77 \\
42. 61 training duration v2 / epochs 002 & 8 & 64 & 64 & 128 & 0.04 & 9.91 & 1.08e-14 & 1.25 \\
43. 61 training duration v2 / epochs 010 & 8 & 64 & 64 & 128 & 0.0392 & 4.3 & 1.34e-14 & 0.803 \\
44. 61 training duration v2 / epochs 025 & 8 & 64 & 64 & 128 & 0.0405 & 4.04 & 1.42e-14 & 1.67 \\
45. 61 training duration v2 / epochs 050 & 8 & 64 & 64 & 128 & 0.0405 & 2.86 & 1.50e-14 & 1.12 \\
46. 61 training duration v2 / epochs 100 & 8 & 64 & 64 & 128 & 0.0404 & 1.56 & 1.63e-14 & 0.77 \\
47. 71 model capacity v2 / hidden 016 & 8 & 64 & 64 & 128 & 0.039 & 0.0548 & 1.52e-14 & 0.0633 \\
48. 71 model capacity v2 / hidden 032 & 8 & 64 & 64 & 128 & 0.0401 & 0.206 & 1.18e-14 & 0.0467 \\
49. 71 model capacity v2 / hidden 064 & 8 & 64 & 64 & 128 & 0.0404 & 1.56 & 1.63e-14 & 0.77 \\
50. 71 model capacity v2 / layers 2 & 8 & 64 & 64 & 128 & 0.0404 & 0.363 & 1.57e-14 & 0.265 \\
51. 71 model capacity v2 / layers 3 & 8 & 64 & 64 & 128 & 0.0404 & 1.56 & 1.63e-14 & 0.77 \\
52. 71 model capacity v2 / layers 4 & 8 & 64 & 64 & 128 & 0.0403 & 0.0136 & 1.08e-14 & 5.25e-03 \\
53. 81 loss weights v2 / conservation 0p0 & 8 & 64 & 64 & 128 & 0.0404 & 2.43 & 1.01e-14 & 0.582 \\
54. 81 loss weights v2 / conservation 0p1 & 8 & 64 & 64 & 128 & 0.0404 & 1.56 & 1.63e-14 & 0.77 \\
55. 81 loss weights v2 / conservation 10p0 & 8 & 64 & 64 & 128 & 0.0405 & 0.28 & 2.41e-14 & 0.0393 \\
56. 81 loss weights v2 / conservation 1p0 & 8 & 64 & 64 & 128 & 0.0403 & 0.298 & 1.68e-14 & 0.0153 \\
57. 81 loss weights v2 / positivity 0p0 & 8 & 64 & 64 & 128 & 0.214 & 3.91 & 2.28e-14 & 2.95 \\
58. 81 loss weights v2 / positivity 0p1 & 8 & 64 & 64 & 128 & 0.214 & 3.91 & 2.28e-14 & 2.95 \\
59. 81 loss weights v2 / positivity 10p0 & 8 & 64 & 64 & 128 & 0.214 & 3.91 & 2.28e-14 & 2.95 \\
60. 81 loss weights v2 / positivity 1p0 & 8 & 64 & 64 & 128 & 0.214 & 3.91 & 2.28e-14 & 2.95 \\
61. 82 positivity activation v3 / positivity 0p0 & 8 & 64 & 64 & 128 & 2.52 & 0.446 & 4.26e-14 & 0.0206 \\
62. 82 positivity activation v3 / positivity 0p1 & 8 & 64 & 64 & 128 & 2.52 & 0.278 & 4.26e-14 & 0.0124 \\
63. 82 positivity activation v3 / positivity 10p0 & 8 & 64 & 64 & 128 & 2.52 & 5.69 & 4.26e-14 & 4.7 \\
64. 82 positivity activation v3 / positivity 1p0 & 8 & 64 & 64 & 128 & 2.52 & 0.45 & 4.26e-14 & 0.261 \\
\bottomrule
\end{longtable}
\normalsize

